Control and Trajectory Optimization for Soft Aerial Manipulation

Manipulation and grasping with unmanned aerial vehicles (UAVs) currently require accurate positioning and are often executed at reduced speed to ensure successful grasps. This is due to the fact that typical UAVs can only accommodate rigid manipulators with few degrees of freedom, which limits their capability to compensate for disturbances caused by the vehicle positioning errors. Moreover, UAVs have to minimize external contact forces in order to maintain stability. Biological systems, on the other hand, exploit softness to overcome similar limitations, and leverage compliance to enable aggressive grasping. This paper investigates control and trajectory optimization for a soft aerial manipulator, consisting of a quadrotor and a tendon-actuated soft gripper, in which the advantages of softness can be fully exploited. To the best of our knowledge, this is the first work at the intersection between soft manipulation and UAV control. We present a decoupled approach for the quadrotor and the soft gripper, combining (i) a geometric controller and a minimum-snap trajectory optimization for the quadrotor (rigid) base, with (ii) a quasi-static finite element model and control-space interpolation for the soft gripper. We prove that the geometric controller asymptotically stabilizes the quadrotor velocity and attitude despite the addition of the soft load. Finally, we evaluate the proposed system in a realistic soft dynamics simulator, and show that: (i) the geometric controller is fairly insensitive to the soft payload, (ii) the platform can reliably grasp unknown objects despite inaccurate positioning and initial conditions, and (iii) the decoupled controller is amenable for real-time execution.

==> tex/extended_abstract.tex <==
%!TEX root = ../main.tex

\newcommand{\myhspace}{\hspace{0mm}}
\newcommand{\mpw}{4.2cm}
\newcommand{\myRate}{1}

We investigate control and trajectory optimization for a soft aerial manipulator, consisting of a quadrotor and a tendon-actuated soft gripper, which for the first time fully brings the advantages of softness to aerial manipulation. 

Manipulation and grasping with unmanned aerial vehicles (UAVs) currently require accurate positioning and are often executed at reduced speed to ensure successful grasps. This is due to the fact that typical UAVs can only accommodate rigid manipulators with few degrees of freedom, which limits their capability to compensate for disturbances caused by vehicle positioning errors or interactions with the environment. Moreover, underactuated aerial platforms have to minimize external contact forces in order to maintain stability. Biological systems, on the other hand, utilize softness to overcome similar limitations and fully exploit compliance to enable aggressive grasping. 

The recent literature in aerial manipulation bears witness to an increasing interest in compliant and underactuated manipulation (\cite{Backus14iros}, \cite{Thomas14bioinspiration}, \cite{Ramon19iros}). However, man-made aerial platforms have hitherto limited the use of soft materials to cases where passive degrees of freedom can be limited or ignored entirely for the purposes of control and planning. Soft systems in general possess infinite passive degrees of freedom, cannot be modeled in closed form and are not differentially flat, putting them at odds with typical techniques for UAV control. The emerging discipline of soft robotics has developed principled approaches to allow control of these systems, opening a new frontier in manipulation. Our work extends these techniques to the aerial domain. To the best of our knowledge, this is the first work at the intersection between soft manipulation and UAV control and planning. 

We present a decoupled approach for soft aerial manipulation, combining 
(i) an adaptive geometric controller and a minimum-snap trajectory optimization for the quadrotor (rigid) base, with 
(ii) a quasi-static finite element model and control-space interpolation for the soft gripper.
Our platform (Fig.~\ref{fig:timelapse}) comprises the frame of a standard quadrotor with the (rigid and heavy) landing gear replaced by a soft gripper.
The gripper consists of four soft fingers, each attached to the quadrotor base and actuated with two pairs of tendons on opposite sides (Fig.~\ref{fig:finger}).

\begin{figure}[t]
\vspace{-5mm}
    \centering
    \includegraphics[width=3in]{timelapse.PNG}
    \caption{We investigate control and trajectory optimization for a \emph{soft aerial manipulator}, consisting of a quadrotor (yellow frame with propeller thrusts in magenta) and a tendon-actuated soft gripper (cyan). The figure shows a temporal sequence leading to a successful grasp in a realistic soft dynamics simulator. \label{fig:timelapse}\vspace{-6mm}}  
\end{figure}

\begin{figure}[b]
    \begin{minipage}{\textwidth}
    \begin{tabular}{cc}%
    \myhspace \hspace{-3mm}
            \begin{minipage}{1.5cm}%
            \centering \vspace{-0.8cm}
            (a) Top view \vspace{1.2cm}\\
            (b) Side view
            \end{minipage}
        &  \hspace{-3mm}
            \begin{minipage}{7cm}%
            \centering%
            \includegraphics[width=0.8\textwidth]{finger.PNG} 
            \end{minipage}
        \end{tabular}
        \vspace{-3mm}
    \end{minipage}
    %\centering
    %\includegraphics[width=.4\textwidth]{finger.PNG}
    \caption{Soft finger with two pairs of tendons on opposite sides. Tendons (black) pass through a set of nodes (red) attached to the finger, such that pulling a tendon causes a contraction of the finger.\label{fig:finger} \vspace{-7mm}}
\end{figure}

Our manipulator is tasked with grasping an object of unknown shape lying over an unknown surface: 
the system is only provided with the centroid of the object. 
We assume we can measure the full state of the quadrotor (its 3D pose and linear and angular velocities) while we operate the soft gripper in open loop (\ie our approach does not need to measure the state of the gripper). 
In particular, we are interested in computing a trajectory of state variables over time and developing a control law that can track the computed trajectory to ensure
a successful grasp in the face of external disturbances. 
While our goal is to simultaneously obtain trajectories and controllers for the soft gripper and the rigid quadrotor, we implement a decoupled approach that implements separate planners/controllers for both subsystems. First, we solve the {\bf drone control subproblem}, 
where we look for an optimal minimum-snap quadrotor trajectory (\cite{Mellinger11icra}) to be tracked by an adaptive geometric controller (\cite{Bisheban20cst}) while treating the soft payload as an unknown disturbance; we show formally that even a non-adaptive geometric controller (\cite{Lee10cdc-geometricControl}) asymptotically stabilizes the quadrotor velocity and attitude despite the addition of a symmetric soft load and wind drag, given limits on the orientation error (technical results and proofs are given in the preprint~\cite{Fishman20arxiv-softDrone}). In practice we relax the symmetry condition, necessitating a controller which can adapt to unmodeled torques.

\begin{figure}
    \begin{center}
    \begin{minipage}{\textwidth}
    \begin{tabular}{cc}%
    \myhspace \hspace{-3mm}
            \begin{minipage}{\mpw}%
            \centering%
            \includegraphics[trim=0mm 0mm 0mm 5mm, clip,height=2.7cm]{adaptive_grasp1.PNG} \\
            \hspace{0cm}(a) 
            \end{minipage}
        & \myhspace 
            \begin{minipage}{\mpw}%
            \centering%
            \includegraphics[trim=0mm 0mm 0mm 5mm, clip,height=2.7cm]{adaptive_grasp2.PNG} \\
            \hspace{0cm}(b) 
            \end{minipage}
        \end{tabular}
    \end{minipage}
    \vspace{-2mm} 
    \caption{Morphological computation refers to the ability of a physical system to supplement explicit control. Here, we show our soft gripper achieving successful grasps despite significant variations in the quadrotor position; the gripper command is the same in (a)-(b).\label{fig:adaptive_grasp}\vspace{-7mm} }
    \end{center}
\end{figure}


Given the quadrotor base trajectory we solve the {\bf soft-gripper control subproblem}, where we look for an optimal control action for the tendon rest lengths. We assume that the soft gripper is \emph{quasi-static}, \ie there is an instantaneous relation between rest lengths and gripper configuration, and approximate the infinite-dimensional soft gripper configurationas a set of  discrete nodes, as in \emph{finite element methods} (FEM). With these, we can find the tendon rest lengths that yield a static node configuration minimizing some objective (\cite{Bern17iros}).
Choosing keyframes along the trajectory, we postulate gripper configurations most likely to yield an enveloping grasp of an object of unknown shape and solve for tendon lengths which yield them. Tendon lengths are linearly interpolated between keyframes; this minimizes the maximum rate of change of tendon lengths, preventing large forces on the tendon attachment points. 

Finally, we evaluate the proposed system in SOFA (~\cite{Faure12sofaam}, ~\cite{Coevoet17advancedrobotics}), a popular soft dynamics simulator. We choose realistic model parameters and show experimentally that the adaptive geometric controller is fairly insensitive to the soft gripper, converging to a target position within 5 seconds while bearing soft payloads ranging in mass by 5 orders of magnitude (Fig.~\ref{fig:geometric_error_densities}).
We demonstrate our platform's ability to reliably execute aggresive grasps on unknown objects despite inaccurate positioning and initial conditions (Fig.~\ref{fig:adaptive_grasp}), moving at velocities of up to 0.5 m/s. 
Finally, we show that the decoupled controller is amenable for real-time execution, with offline trajectory planning taking~$\sim1$ second and online control calculation in milliseconds.

\begin{figure}[b]
\centering
\includegraphics[width=.52\textwidth]{geometric_error_densities_adaptive.png}
\caption{Mean and standard deviation of the tracking errors for soft gripper densities $\{10^{-2}, 10^3, 10^4\} \SI{}{kg/m^3}$. Statistics are computed over 20 runs with randomly chosen target locations on the unit circle.\label{fig:geometric_error_densities}\vspace{-3mm}}
\end{figure}

Ongoing work includes real implementation and testing of the soft aerial manipulator proposed in this paper.
More fundamentally, we are investigating the proposed ``soft drone'' design for other applications, including aggressive landing, perching, and collision-resistant navigation. 

\textbf{Video Attachment: {\color{blue} https://youtu.be/NNpQxP0SPFk}}

==> tex/graspPlan.tex <==
%!TEX root = ../main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

